3D Shape Reconstruction from Vision and Touch

When a toddler is presented a new toy, their instinctual behaviour is to pick it upand inspect it with their hand and eyes in tandem, clearly searching over its surface to properly understand what they are playing with. At any instance here, touch provides high fidelity localized information while vision provides complementary global context. However, in 3D shape reconstruction, the complementary fusion of visual and haptic modalities remains largely unexplored. In this paper, we study this problem and present an effective chart-based approach to multi-modal shape understanding which encourages a similar fusion vision and touch information.To do so, we introduce a dataset of simulated touch and vision signals from the interaction between a robotic hand and a large array of 3D objects. Our results show that (1) leveraging both vision and touch signals consistently improves single-modality baselines; (2) our approach outperforms alternative modality fusion methods and strongly benefits from the proposed chart-based structure; (3) there construction quality increases with the number of grasps provided; and (4) the touch information not only enhances the reconstruction at the touch site but also extrapolates to its local neighborhood.

==> 3_Problem_Setup.tex <==
We consider the problem of 3D shape reconstruction from visual and haptic signals. We assume that visual information is obtained from a single RGB image and haptic information is obtained from gel-based touch sensors with high spatial resolution, such as a GelSight sensor \cite{GelSight}.
More precisely, let $V$ denote the RGB image used as vision signal. Let $T = [R_i, P_i]_{i=1}^{n_t}$ denote the touch information, where $R_i$ is one touch sensor reading, $P_i$ its corresponding position and rotation in space, and $n_t$ is the number of touch sensors. Let $O$ be the target object shape, represented as a surface mesh. The objective is to learn a function $f_{\theta}$ parameterized by $\theta$ that predicts an object shape reconstruction $\hat{O} = f_{\theta}(V, T)$, also represented as surface mesh, such that it best captures the surface defined by $O$. 

We represent the surfaces $\hat O$ as a set of independent surfaces, $\{C_i\}_{i=1}^{n_c}$, called charts \emph{charts}. A chart, $C_i$, is implemented as a planar, triangular, 3D polygon mesh, composed of connected triangular faces, each defined by 3 vertex positions. Figure~\ref{fig:Chart_Diagram} depicts the structure of a chart, and outlines how a set of charts can combined to form a closed 3D surface.







